On Freeze LTL with Ordered Attributes

This paper is concerned with Freeze LTL, a temporal logic on data words with registers. In a (multi-attributed) data word each position carries a letter from a finite alphabet and assigns a data value to a fixed, finite set of attributes. The satisfiability problem of Freeze LTL is undecidable if more than one register is available or tuples of data values can be stored and compared arbitrarily. Starting from the decidable one-register fragment we propose an extension that allows for specifying a dependency relation on attributes. This restricts in a flexible way how collections of attribute values can be stored and compared. This conceptual dimension is orthogonal to the number of registers or the available temporal operators. The extension is strict. Admitting arbitrary dependency relations satisfiability becomes undecidable. Tree-like relations, however, induce a family of decidable fragments escalating the ordinal-indexed hierarchy of fast-growing complexity classes, a recently introduced framework for non-primitive recursive complexities. This results in completeness for the class ${\bf F}_{\epsilon_0}$. We employ nested counter systems and show that they relate to the hierarchy in terms of the nesting depth.

==> fig_threads2.tex <==
\begin{tikzpicture}[
    level 1/.style={level distance =2.5em},
    level 2/.style={level distance =2.5em},
    level 3/.style={level distance =2.5em},
    >=stealth
  ]
  
  \path 
  node (root) {$\st$} 
     child [sibling distance =8em]{node {$｛φ_3, ↑^1｝\ \cmark$}
      child { node {$｛φ_2｝$}
        child {node {$｛φ_1,φ_3｝$}}
      }
      child [sibling distance =3em]{ node {$｛↑^1, ↑^2｝\ \cmark$}
        child {node {$｛φ_2｝$}}
        child {node {$｛｝\ \cmark$}}
      }
    } 
    child {node {$｛↓^1φ_3｝$} child {node {$｛φ_1,φ_2｝$} child {node {$｛φ_3｝$}}}};
  
\end{tikzpicture}


==> macros_todo.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Macros for marking multiple lines of text - remove for final version %%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{atbegshi}
\usepackage{refcount}
\usepackage{setspace}
\usepackage{tikzpagenodes}
\usetikzlibrary{calc}

\newcounter{bordercntr}
\newcounter{borderpages}

\newcommand\tikzmark[1]{%
  \tikz[overlay,remember picture] \node[inner xsep=0pt] (#1) {};}

\newenvironment{ltodo}[2][7pt]
{%
  \gdef\borderspacing{#1}
  \stepcounter{bordercntr}%
  \tikzmark{start-border}\label{start-border\thebordercntr}%
  \tikz[remember picture,overlay]
    \node[anchor=north west,inner sep=0pt,text=red,font=\footnotesize] at 
  ([xshift=\marginparsep,yshift=0.65ex]current page text area.east|-start-border.north)
  {\parbox{\marginparwidth}{\begin{spacing}{0.8}\raggedright#2\end{spacing}}};%
  % if the marks are in the same page, nothing is done
  % otherwise, the decoration is drawn from the starting point to the page bottom
  % and, if necessary, intermediate pages will also receive the decoration
  \ifnum\getpagerefnumber{start-border\thebordercntr}=\getpagerefnumber{end-border\thebordercntr}\else
    \begin{tikzpicture}[overlay, remember picture]
      % corner points
      \path ([xshift=0.7ex,yshift=1.25ex]current page text area.east|-start-border.north) node (tr) {};
      \path ([xshift=-0.7ex,yshift=1.25ex]current page text area.west|-start-border.north) node (tl) {};    
      \path ([xshift=0.7ex, yshift=-1ex]current page text area.south east) node (br) {};
      \path ([xshift=-0.7ex, yshift=-1ex]current page text area.south west) node (bl) {};
      % shape 
      \path[draw, rounded corners] (bl.center) -- (tl.center) -- (tr.center) -- (br.center);
      \path[fill=orange, opacity=0.2, rounded corners] (bl.center) -- (tl.center) -- (tr.center) -- (br.center);
    \end{tikzpicture}%
\setcounter{borderpages}{\numexpr\getpagerefnumber{end-border\thebordercntr}-\getpagerefnumber{start-border\thebordercntr}}%
    \ifnum\value{borderpages}>1\relax
      \AtBeginShipoutNext{\tikzborderpage[#1]}%
    \fi%
  \fi%
\ignorespaces%
}
{\tikzmark{end-border}\label{end-border\thebordercntr}%
  % if the marks are in the same page, the decoration is drawn
  % otherwise, the decoration is drawn from the top of the page to the end mark
  \ifnum\getpagerefnumber{start-border\thebordercntr}=\getpagerefnumber{end-border\thebordercntr}%
    \begin{tikzpicture}[overlay, remember picture]
      % corner points
      \path ([xshift=0.7ex,yshift=.5em]current page text area.east|-start-border.north) node (tr) {};
      \path ([xshift=-0.7ex,yshift=0.5em]current page text area.west|-start-border.north) node (tl) {};    
      \path ([xshift=0.7ex,yshift=0.1em]current page text area.east|-end-border.south) node (br) {};
      \path ([xshift=-0.7ex, yshift=0.1em]current page text area.west|-end-border.south) node (bl) {};
      % shape 
%      \path[draw, rounded corners] (bl.center) -- (tl.center) -- (tr.center) -- (br.center) -- (bl.center);
%      \path[fill=red, opacity=0.5, rounded corners] (bl.center) -- (tl.center) -- (tr.center) -- (br.center) -- (bl.center);
      \path[fill=orange, opacity=0.2, rounded corners] (tl.center) rectangle (br.center);
      \path[draw=black, rounded corners] (tl.center) rectangle (br.center);

    \end{tikzpicture}%
  \else
    \begin{tikzpicture}[overlay, remember picture]
      % corner points
      \path ([xshift=0.7ex,yshift=0]current page text area.east|-end-border.south) node (br) {};
      \path ([xshift=-0.7ex,yshift=0]current page text area.west|-end-border.south) node (bl) {};    
      \path ([xshift=0.7ex, yshift=1.25ex]current page text area.north east) node (tr) {};
      \path ([xshift=-0.7ex, yshift=1.25ex]current page text area.north west) node (tl) {};

      % shape 
      \path[draw, rounded corners] (tl.center) -- (bl.center) -- (br.center) -- (tr.center);
      \path[fill=orange, opacity=0.2, rounded corners] (tl.center) -- (bl.center) -- (br.center) -- (tr.center);
    \end{tikzpicture}%
  \fi%
}

\newenvironment{lidea}[2][7pt]
{%
  \gdef\borderspacing{#1}
  \stepcounter{bordercntr}%
  \tikzmark{start-border}\label{start-border\thebordercntr}%
  \tikz[remember picture,overlay]
    \node[anchor=north west,inner sep=0pt,text={green!50!black},font=\footnotesize] at 
  ([xshift=\marginparsep,yshift=0.65ex]current page text area.east|-start-border.north)
  {\parbox{\marginparwidth}{\begin{spacing}{0.8}\raggedright#2\end{spacing}}};%
  % if the marks are in the same page, nothing is done
  % otherwise, the decoration is drawn from the starting point to the page bottom
  % and, if necessary, intermediate pages will also receive the decoration
  \ifnum\getpagerefnumber{start-border\thebordercntr}=\getpagerefnumber{end-border\thebordercntr}\else
    \begin{tikzpicture}[overlay, remember picture]
      % corner points
      \path ([xshift=0.7ex,yshift=1.25ex]current page text area.east|-start-border.north) node (tr) {};
      \path ([xshift=-0.7ex,yshift=1.25ex]current page text area.west|-start-border.north) node (tl) {};    
      \path ([xshift=0.7ex, yshift=-1ex]current page text area.south east) node (br) {};
      \path ([xshift=-0.7ex, yshift=-1ex]current page text area.south west) node (bl) {};
      % shape 
      \path[draw, rounded corners] (bl.center) -- (tl.center) -- (tr.center) -- (br.center);
      \path[fill=green, opacity=0.2, rounded corners] (bl.center) -- (tl.center) -- (tr.center) -- (br.center);
    \end{tikzpicture}%
\setcounter{borderpages}{\numexpr\getpagerefnumber{end-border\thebordercntr}-\getpagerefnumber{start-border\thebordercntr}}%
    \ifnum\value{borderpages}>1\relax
      \AtBeginShipoutNext{\tikzborderpage[#1]}%
    \fi%
  \fi%
\ignorespaces%
}
{\tikzmark{end-border}\label{end-border\thebordercntr}%
  % if the marks are in the same page, the decoration is drawn
  % otherwise, the decoration is drawn from the top of the page to the end mark
  \ifnum\getpagerefnumber{start-border\thebordercntr}=\getpagerefnumber{end-border\thebordercntr}%
    \begin{tikzpicture}[overlay, remember picture]
      % corner points
      \path ([xshift=0.7ex,yshift=.5em]current page text area.east|-start-border.north) node (tr) {};
      \path ([xshift=-0.7ex,yshift=0.5em]current page text area.west|-start-border.north) node (tl) {};    
      \path ([xshift=0.7ex,yshift=0.1em]current page text area.east|-end-border.south) node (br) {};
      \path ([xshift=-0.7ex, yshift=0.1em]current page text area.west|-end-border.south) node (bl) {};
      % shape 
%      \path[draw, rounded corners] (bl.center) -- (tl.center) -- (tr.center) -- (br.center) -- (bl.center);
%      \path[fill=red, opacity=0.5, rounded corners] (bl.center) -- (tl.center) -- (tr.center) -- (br.center) -- (bl.center);
      \path[fill=green, opacity=0.2, rounded corners] (tl.center) rectangle (br.center);
      \path[draw=black, rounded corners] (tl.center) rectangle (br.center);

    \end{tikzpicture}%
  \else
    \begin{tikzpicture}[overlay, remember picture]
      % corner points
      \path ([xshift=0.7ex,yshift=0]current page text area.east|-end-border.south) node (br) {};
      \path ([xshift=-0.7ex,yshift=0]current page text area.west|-end-border.south) node (bl) {};    
      \path ([xshift=0.7ex, yshift=1.25ex]current page text area.north east) node (tr) {};
      \path ([xshift=-0.7ex, yshift=1.25ex]current page text area.north west) node (tl) {};

      % shape 
      \path[draw, rounded corners] (tl.center) -- (bl.center) -- (br.center) -- (tr.center);
      \path[fill=green, opacity=0.2, rounded corners] (tl.center) -- (bl.center) -- (br.center) -- (tr.center);
    \end{tikzpicture}%
  \fi%
}


\newenvironment{deprecated}[2][7pt]
{%
  \gdef\borderspacing{#1}
  \stepcounter{bordercntr}%
  \tikzmark{start-border}\label{start-border\thebordercntr}%
  \tikz[remember picture,overlay]
    \node[anchor=north west,inner sep=0pt,text=red,font=\footnotesize] at 
  ([xshift=\marginparsep,yshift=0.65ex]current page text area.east|-start-border.north)
  {\parbox{\marginparwidth}{\begin{spacing}{0.8}\raggedright#2\end{spacing}}};%
  % if the marks are in the same page, nothing is done
  % otherwise, the decoration is drawn from the starting point to the page bottom
  % and, if necessary, intermediate pages will also receive the decoration
  \ifnum\getpagerefnumber{start-border\thebordercntr}=\getpagerefnumber{end-border\thebordercntr}\else
    \begin{tikzpicture}[overlay, remember picture]
      % corner points
      \path ([xshift=0.7ex,yshift=1.25ex]current page text area.east|-start-border.north) node (tr) {};
      \path ([xshift=-0.7ex,yshift=1.25ex]current page text area.west|-start-border.north) node (tl) {};    
      \path ([xshift=0.7ex, yshift=-1ex]current page text area.south east) node (br) {};
      \path ([xshift=-0.7ex, yshift=-1ex]current page text area.south west) node (bl) {};
      % shape 
      \path[draw, rounded corners] (bl.center) -- (tl.center) -- (tr.center) -- (br.center);
      \path[fill=yellow, opacity=0.2, rounded corners] (bl.center) -- (tl.center) -- (tr.center) -- (br.center);
    \end{tikzpicture}%
\setcounter{borderpages}{\numexpr\getpagerefnumber{end-border\thebordercntr}-\getpagerefnumber{start-border\thebordercntr}}%
    \ifnum\value{borderpages}>1\relax
      \AtBeginShipoutNext{\tikzborderpage[#1]}%
    \fi%
  \fi%
\ignorespaces%
}
{\tikzmark{end-border}\label{end-border\thebordercntr}%
  % if the marks are in the same page, the decoration is drawn
  % otherwise, the decoration is drawn from the top of the page to the end mark
  \ifnum\getpagerefnumber{start-border\thebordercntr}=\getpagerefnumber{end-border\thebordercntr}%
    \begin{tikzpicture}[overlay, remember picture]
      % corner points
      \path ([xshift=0.7ex,yshift=.5em]current page text area.east|-start-border.north) node (tr) {};
      \path ([xshift=-0.7ex,yshift=0.5em]current page text area.west|-start-border.north) node (tl) {};    
      \path ([xshift=0.7ex,yshift=0.1em]current page text area.east|-end-border.south) node (br) {};
      \path ([xshift=-0.7ex, yshift=0.1em]current page text area.west|-end-border.south) node (bl) {};
      % shape 
%      \path[draw, rounded corners] (bl.center) -- (tl.center) -- (tr.center) -- (br.center) -- (bl.center);
%      \path[fill=red, opacity=0.5, rounded corners] (bl.center) -- (tl.center) -- (tr.center) -- (br.center) -- (bl.center);
      \path[fill=yellow, opacity=0.2, rounded corners] (tl.center) rectangle (br.center);
      \path[draw=black, rounded corners] (tl.center) rectangle (br.center);

    \end{tikzpicture}%
  \else
    \begin{tikzpicture}[overlay, remember picture]
      % corner points
      \path ([xshift=0.7ex,yshift=0]current page text area.east|-end-border.south) node (br) {};
      \path ([xshift=-0.7ex,yshift=0]current page text area.west|-end-border.south) node (bl) {};    
      \path ([xshift=0.7ex, yshift=1.25ex]current page text area.north east) node (tr) {};
      \path ([xshift=-0.7ex, yshift=1.25ex]current page text area.north west) node (tl) {};

      % shape 
      \path[draw, rounded corners] (tl.center) -- (bl.center) -- (br.center) -- (tr.center);
      \path[fill=yellow, opacity=0.2, rounded corners] (tl.center) -- (bl.center) -- (br.center) -- (tr.center);
    \end{tikzpicture}%
  \fi%
}


\newenvironment{sidemark}[2][7pt]
{%
  \gdef\borderspacing{#1}
  \stepcounter{bordercntr}%
  \tikzmark{start-border}\label{start-border\thebordercntr}%
  \tikz[remember picture,overlay]
    \node[anchor=north west,inner sep=0pt,text=red,font=\footnotesize] at 
  ([xshift=\marginparsep,yshift=0.65ex]current page text area.east|-start-border.north)
  {\parbox{\marginparwidth}{\begin{spacing}{0.8}\raggedright#2\end{spacing}}};%
  % if the marks are in the same page, nothing is done
  % otherwise, the decoration is drawn from the starting point to the page bottom
  % and, if necessary, intermediate pages will also receive the decoration
  \ifnum\getpagerefnumber{start-border\thebordercntr}=\getpagerefnumber{end-border\thebordercntr}\else
    \begin{tikzpicture}[overlay, remember picture]
    \draw [ultra thick,red]
         ([xshift=\borderspacing,yshift=0.65ex]current page text area.east|-start-border.north) --  
         ([xshift=\borderspacing]current page text area.south east);
    \end{tikzpicture}%
\setcounter{borderpages}{\numexpr\getpagerefnumber{end-border\thebordercntr}-\getpagerefnumber{start-border\thebordercntr}}%
    \ifnum\value{borderpages}>1\relax
      \AtBeginShipoutNext{\tikzborderpage[#1]}%
    \fi%
  \fi%
\ignorespaces%
}
{\tikzmark{end-border}\label{end-border\thebordercntr}%
  % if the marks are in the same page, the decoration is drawn
  % otherwise, the decoration is drawn from the top of the page to the end mark
  \ifnum\getpagerefnumber{start-border\thebordercntr}=\getpagerefnumber{end-border\thebordercntr}%
    \begin{tikzpicture}[overlay, remember picture]
    \draw [ultra thick,red]
         ([xshift=\borderspacing,yshift=0.65ex]current page text area.east|-start-border.north) --  
         ([xshift=\borderspacing,yshift=0.65ex]current page text area.east|-end-border.south);
    \end{tikzpicture}%
  \else
    \begin{tikzpicture}[overlay, remember picture]
    \draw [ultra thick,red]
         ([xshift=\borderspacing]current page text area.north east) --  
         ([xshift=\borderspacing,yshift=0.65ex]current page text area.east|-end-border.south);
    \end{tikzpicture}%
  \fi%
}

% the command to draw the decoration in intermediate pages from the top
% to the bottom of the page
\newcommand\tikzborderpage[1][0pt]{%
  \begin{tikzpicture}[overlay, remember picture]
    %corner points
    \path ([xshift=0.7ex, yshift=1.25ex]current page text area.north east) node (tr) {};
    \path ([xshift=-0.7ex, yshift=1.25ex]current page text area.north west) node (tl) {};
    \path ([xshift=0.7ex, yshift=-1ex]current page text area.south east) node (br) {};
    \path ([xshift=-0.7ex, yshift=-1ex]current page text area.south west) node (bl) {};
  
    \path[fill=orange, opacity=0.2] (tl.center) rectangle (br.center);
    \path[draw=black] (tl.center) -- (bl.center);
    \path[draw=black] (tr.center) -- (br.center);

  
%    \draw[ultra thick,gray]
%         ([xshift=\borderspacing,yshift=-\baselineskip]current page text area.north east) --  
%         ([xshift=\borderspacing,yshift=0.65ex]current page text area.south east);
  \end{tikzpicture}
  \addtocounter{borderpages}{-1}%
  \ifnum\value{borderpages}>1
    \AtBeginShipoutNext{\tikzborderpage[#1]}%
  \fi%
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

